Parametric Design of Underwater Optical Systems

The design of optical systems for underwater vehicles is a complex process where the selection of cameras, lenses, housings, and operational parameters greatly influence the performance of the complete system. Determining the correct combination of components and parameters for a given set of operational requirements is currently a process based on trial and error as well as the specialized knowledge and experience of the designer. In this paper, we introduce an open-source tool for the parametric exploration of the design space of underwater optical systems and review the most significant underwater light effects with the corresponding models to estimate the response and performance of the complete imaging system.

==> text/background.tex <==






%Akkaynak et al~\cite{akkaynak2018revised} present a revised model, describing additional dependencies of the backscattered signal on environment and system parameters.
%In ~\cite{kaeli2017illumination} the authors use an underwater image formation model and \ac{DVL} measurements from an \ac{AUV} to simultaneously correct the color appearance and the illumination artifacts caused by an artificial light beam pattern. 
%Deep learning has also been applied to the underwater color correction problem~ but is currently limited in the resolution of the images\cite{7995024, 7761342}.

%Other applications of underwater image formation models include the estimation of chlorophyll and dissolved organic matter in the water column~\cite{Solonenko:15}, the improvement of structure from motion 3D reconstructions through explicit refraction modelling~\cite{6751116}, the characterization of benthic habitats through measuring reflectivity of the seafloor~\cite{davie_benthic_2008} or the rendering  of artificial underwater images for synthetic data generation~\cite{sedlazeck_simulating_nodate}. 





%Background on lights \\

%Backgrounds on underwater light propagation \\

%Background on reflectance \\ 

%Background on sensor response \\
